A Privacy-Preserving, Accountable and Spam-Resilient Geo-Marketplace

Mobile devices with rich features can record videos, traffic parameters or air quality readings along user trajectories. Although such data may be valuable, users are seldom rewarded for collecting them. Emerging digital marketplaces allow owners to advertise their data to interested buyers. We focus on geo-marketplaces, where buyers search data based on geo-tags. Such marketplaces present significant challenges. First, if owners upload data with revealed geo-tags, they expose themselves to serious privacy risks. Second, owners must be accountable for advertised data, and must not be allowed to subsequently alter geo-tags. Third, such a system may be vulnerable to intensive spam activities, where dishonest owners flood the system with fake advertisements. We propose a geo-marketplace that addresses all these concerns. We employ searchable encryption, digital commitments, and blockchain to protect the location privacy of owners while at the same time incorporating accountability and spam-resilience mechanisms. We implement a prototype with two alternative designs that obtain distinct trade-offs between trust assumptions and performance. Our experiments on real location data show that one can achieve the above design goals with practical performance and reasonable financial overhead.

==> references-old <==
@String{ tods   = "{ACM} {TODS}"}
@String{ ieeetc = "{IEEE} {Trans. on Computers}"}
@String{ vldb   = "Proceedings of International Conference on Very Large Data Bases (VLDB)"}
@String{ mobide = "Proc. of {ACM} Int. Workshop on Data Engineering for Wireless and Mobile Access"}
@String{ ssd    = "Proc. of {SSD}"}
@String{ cidr   = "Proc. of Biennial Conference on Innovative Data Systems Research"}
@String{ tkde   = "{IEEE} Transactions on Knowledge and Data Engineering (TKDE)"}
@String{ mdm    = "Proc. of {MDM}"}
@String{ ssdbm  = "Proc. of {SSDBM} Conf."}
@String{ ideas  = "Proc. of Int. Database Engineering and Applications Symposium"}
@String{ kdd    = "Proc. of {KDD}"}
@String{ edbt   = "Proc. of {EDBT} Conf."}
@String{ sstd   = "Proceedings of International Symposium on Spatial and Temporal Databases (SSTD)"}
@String{ sigmod = "Proceedings of International Conference on Management of Data (ACM SIGMOD)"}
@String{ dexa   = "Proc. of {DEXA}"}
@String{ acmcs  = "{ACM} Computing Surveys"}
@String{ cacm   = "Communications of the {ACM}"}
@String{ tocs   = "{IEEE} Transactions on Computers"}
@String{ ijcai  = "Proc. of {IJCAI}"}
@String{ icde   = "Proceedings of International Conference on Data Engineering (ICDE)"}
@String{ cikm   = "Proc. of {CIKM}"}
@String{ icdm   = "Proc. of {ICDM}"}
@String{ acmgis = "Proceedings of International Conference on Advances in Geographic Information Systems (ACM SIGSPATIAL GIS)"}
@String{ icdt   = "Proc. of {ICDT}"}
@String{ icdcs  = "Proc. of {ICDCS}"}
@String{ pods   = "Proc. of {ACM} {PODS}"}
@String{ mobisys = "Proc. of {USENIX} {MobiSys}"}
@String{ www    = "Proc. of Int. Conference on World Wide Web (WWW)"}

@article{prov_survey,
 author = {Simmhan, Yogesh L. and Plale, Beth and Gannon, Dennis},
 title = {A survey of data provenance in e-science},
 journal = {SIGMOD Rec.},
 issue_date = {September 2005},
 volume = {34},
 number = {3},
 month = sep,
 year = {2005},
 pages = {31--36}
} 

@INPROCEEDINGS{Chen_Acs_Castelluccia_2012,
  AUTHOR =       {Chen, Rui and Acs, Gergely and Castelluccia, Claude},
  TITLE =        {Differentially private sequential data publication via variable-length n-grams},
  BOOKTITLE =    {ACM CCS},
  YEAR =         {2012},
  pages =        {638--649}
}


@INPROCEEDINGS{cpssy12,
  AUTHOR =       {Graham Cormode and Cecilia Procopiuc and Entong Shen and Divesh Srivastava and Ting Yu},
  TITLE =        {Differentially private spatial decompositions},
  BOOKTITLE =    {ICDE},
  YEAR =         {2012},
  pages = 		{20--31}
}

@inproceedings{calibratingSensitivity,
  author    = {Cynthia Dwork and
               Frank McSherry and
               Kobbi Nissim and
               Adam Smith},
  title     = {Calibrating Noise to Sensitivity in Private Data Analysis},
  booktitle = {TCC},
  year      = {2006},
  pages     = {265-284}
}

@inproceedings{GIM99,
 author = {Aristides Gionis and Piotr Indyk and Rajeev Motwani},
 title = "{Similarity Search in High Dimensions via Hashing}",
 booktitle = vldb,
 year = {1999},
 pages = {518--529}
}

@inproceedings{outlier-det,
 author = {Sridhar Ramaswamy and Rajeev Rastogi and Kyuseok Shim}, 
 title = "{Efficient algorithms for mining outliers from large data sets}",
 booktitle = sigmod,
 year = {2000},
 pages = {427--438}
}

@inproceedings{secureKNN,
 author = {W. K. Wong and D. W. Cheung and B. Kao and N. Mamoulis}, 
 title = "{Secure k-NN Computation on Encrypted Databases}",
 booktitle = sigmod,
 year = {2009},
 pages = {139--152}
}

@manual{Anonymizer,
    AUTHOR       = "",
    TITLE = "http://www.anonymizer.com/"
    }

@manual{Mailshell,
    AUTHOR       = "",
    TITLE = "http://www.mailshell.com/"
    }

@manual{Spamgourmet,
    AUTHOR       = "",
    TITLE = "http://www.spamgourmet.com/"
    }

@manual{Ugc,
    AUTHOR       = "",
    TITLE = "http://www.ugcprinciples.com/"
    }

@manual{Cgm,
    AUTHOR       = "",
    TITLE = "http://www.nielsenbuzzmetrics.com/cgm"
    }

@manual{nist-hash,
    AUTHOR       = "",
    TITLE = "National Institute of Standards and Technology. Secure Hashing. http://csrc.nist.gov/groups/ST/toolkit/secure\_hashing.html"
    }

@inproceedings{sew02,
  author    = {Peter Stuckmann and Niels Ehlers and Bianca Wouters},
  title     = {{GPRS Traffic Performance Measurements}},
  booktitle = {IEEE Vehicular Technology Conference},
  year      = {2002},
}

@inproceedings{as00,
  author    = {Rakesh Agrawal and
               Ramakrishnan Srikant},
  title     = {{Privacy-Preserving Data Mining}},
  booktitle = {SIGMOD},
  year      = {2000},
}

@inproceedings{hdc05,
  author    = {Zhengli Huang and
               Wenliang Du and
               Biao Chen},
  title     = {{Deriving Private Information from Randomized Data}},
  booktitle = {SIGMOD},
  year      = {2005},
}

@article{lkr06,
  author    = {Kun Liu and
               Hillol Kargupta and
               Jessica Ryan},
  title     = {{Random Projection-Based Multiplicative Data Perturbation
               for Privacy Preserving Distributed Data Mining}},
  journal   = {IEEE TKDE},
  volume    = {18},
  number    = {1},
  year      = {2006},
  pages     = {92-106},
}

@article{hs99,
 author = "G. R. Hjaltason and H. Samet",
 title = "{Distance Browsing in Spatial Databases}",
 journal = "TODS",
 volume = "24(2)",
 pages = "265-318",
 year = "1999",
}

@inproceedings{bkss90,
  author    = {N. Beckmann and H.-P. Kriegel and R. Schneider and B. Seeger},
  title     = {{The R*-tree: An Efficient and Robust Access Method for Points and Rectangles}},
  booktitle = {SIGMOD},
  year      = {1990},
}


@inproceedings{in07,
  author    = {Tochukwu Iwuchukwu and
               Jeffrey F. Naughton},
  title     = {{K-Anonymization as Spatial Indexing: Toward Scalable and
               Incremental Anonymization}},
  booktitle = {VLDB},
  year      = {2007},
}


@inproceedings{llv07,
  author    = {Ninghui Li and
               Tiancheng Li and
               Suresh Venkatasubramanian},
  title     = {{t-Closeness: Privacy Beyond k-Anonymity and l-Diversity}},
  booktitle = {ICDE},
  year      = {2007},
}


@article{dgms03,
 author = {Premkumar Devanbu and Michael Gertz and Charles Martel and Stuart G. Stubblebine},
 title = {{Authentic Data Publication over the Internet}},
 journal = {J. Comput. Secur.},
 volume = {11},
 number = {3},
 year = {2003},
 issn = {0926-227X},
 pages = {291--314},
 publisher = {IOS Press},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@article{mjfs01,
  author    = {Bongki Moon and
               H. V. Jagadish and
               Christos Faloutsos and
               Joel H. Saltz},
  title     = {{Analysis of the Clustering Properties of the Hilbert Space-Filling
               Curve}},
  journal   = {IEEE TKDE},
  volume    = {13},
  number    = {1},
  year      = {2001},
  pages     = {124-141}
}


@inproceedings{iw06,
  author    = {Piotr Indyk and
               David P. Woodruff},
  title     = {{Polylogarithmic Private Approximations and Efficient Matching}},
  booktitle = {TCC},
  year      = {2006},
}


@inproceedings{SovJoins,
 author = {Rakesh Agrawal and Dmitri Asonov and Murat Kantarcioglu and Yaping Li},
 title = {Sovereign Joins},
 booktitle = icde,
 year = {2006},
 pages = {26}
 }


@article{crypto04,
 author = {Oded Goldreich},
 title = {{The Foundations of Cryptography, Volume 2}},
 journal = {Cambridge University Press},
 year = {2004},
}

@inproceedings{skk06,
  author    = {Mark Shaneck and
               Yongdae Kim and
               Vipin Kumar},
  title     = {{Privacy Preserving Nearest Neighbor Search}},
  booktitle = {ICDM Workshops},
  year      = {2006},
}


@inproceedings{cpt06,
  author    = {Weiwei Cheng and
               HweeHwa Pang and
               Kian-Lee Tan},
  title     = {{Authenticating Multi-dimensional Query Results in Data Publishing}},
  booktitle = {DBSec},
  year      = {2006},
}

@inproceedings{pjrt05,
  author    = {HweeHwa Pang and
               Arpit Jain and
               Krithi Ramamritham and
               Kian-Lee Tan},
  title     = {{Verifying Completeness of Relational Query Results in Data Publishing}},
  booktitle = {SIGMOD},
  year      = {2005},
}

@inproceedings{merkle89,
  author    = {Ralph C. Merkle},
  title     = {{A Certified Digital Signature}},
  booktitle = {CRYPTO},
  year      = {1989},
}

@inproceedings{lgk06,
  author    = {Kun Liu and
               Chris Giannella and
               Hillol Kargupta},
  title     = {{An Attacker's View of Distance Preserving Maps for Privacy Preserving Data Mining}},
  booktitle = {PKDD},
  year      = {2006},
}

@inproceedings{xt06,
  author    = {Xiaokui Xiao and
               Yufei Tao},
  title     = {{Personalized Privacy Preservation}},
  booktitle = {SIGMOD},
  year      = {2006},
}

@inproceedings{aksx04,
  author    = {Rakesh Agrawal and
               Jerry Kiernan and
               Ramakrishnan Srikant and
               Yirong Xu},
  title     = {{Order-Preserving Encryption for Numeric Data}},
  booktitle = {SIGMOD},
  year      = {2004},
}


@article{b71,
 author = {A. R. Butz},
 title = {{Alternative Algorithm for Hilbert's Space-Filling Curve}},
 journal = {IEEE Trans. Comput.},
 volume = {C-20},
 number = {4},
 year = {1971},
 pages = {424-426},
}

@inproceedings{hmi02,
  author    = {Hakan Hacig{\"u}m{\"u}s and
               Sharad Mehrotra and
               Balakrishna R. Iyer},
  title     = {{Providing Database as a Service}},
  booktitle = {ICDE},
  year      = {2002},
}

@inproceedings{hilm02,
  author    = {Hakan Hacig{\"u}m{\"u}s and
               Balakrishna R. Iyer and
               Chen Li and
               Sharad Mehrotra},
  title     = {{Executing SQL over Encrypted Data in the Database-Service-Provider Model}},
  booktitle = {SIGMOD},
  year      = {2002},
}



@inproceedings{gkr04,
  author    = {Sandeep Gupta and
               Swastik Kopparty and
               Chinya V. Ravishankar},
  title     = {{Roads, Codes and Spatiotemporal Queries}},
  booktitle = {PODS},
  year      = {2004},
}

@inproceedings{ks07,
  author    = {Ali Khoshgozaran and Cyrus Shahabi},
  title     = {{Blind Evaluation of Nearest Neighbor Queries Using Space Transformation to Preserve Location Privacy}},
  booktitle = {SSTD},
  year      = {2007},
}

@inproceedings{acdvs07,
  author    = {Claudio Agostino Ardagna and
               Marco Cremonini and
               Ernesto Damiani and
               Sabrina De Capitani di Vimercati and
               Pierangela Samarati},
  title     = {{Location Privacy Protection Through Obfuscation-Based Techniques}},
  booktitle = {DBSec},
  year      = {2007},
}

@inproceedings{duckham05a,
 author = {Matt Duckham and Lars Kulik},
 title = {{A Formal Model of Obfuscation and Negotiation for Location Privacy}},
 booktitle = {PERVASIVE},
 year = {2005},
}

@inproceedings{kido05,
 author = {H. Kido and Y. Yanagisawa and T. Satoh},
 title = {{An Anonymous Communication Technique using Dummies for Location-based Services}},
 booktitle = {IEEE International Conference on Pervasive Services (ICPS)},
 year = {2005},
}

@article{hl06,
 author = {Haibo Hu and Dik Lun Lee},
 title = {{Range Nearest-Neighbor Query}},
 journal = {IEEE TKDE},
 volume = {18(1)},
 pages = {78-91},
 year = {2006},
}

@inproceedings{gruteser03,
 author = {M. Gruteser and D. Grunwald},
 title = {{Anonymous Usage of Location-Based Services Through Spatial and Temporal Cloaking}},
 booktitle = {USENIX MobiSys},
 year = {2003},
}

@inproceedings{gedik05,
 author = {B. Gedik and L. Liu},
 title = {{Location Privacy in Mobile Systems: A Personalized Anonymization Model}},
 booktitle = {ICDCS},
 year = {2005},
}

@article{gedik08,
 author = {B. Gedik and L. Liu},
 title = {{Protecting Location Privacy with Personalized k-Anonymity: Architecture and Algorithms}},
 journal = {IEEE TMC},
 volume = {7(1)},
 pages = {1-18},
 year = {2008},
}


@article{sweeney02,
 author = {L. Sweeney},
 title = {{$k$-Anonymity: A Model for Protecting Privacy}},
 journal = {International Journal on Uncertainty, Fuzziness and Knowledge-Based Systems},
 volume = {10(5)},
 pages = {557-570},
 year = {2002},
}


@article{dijk59,
    author = "E. W. Dijkstra",
    title = {{A Note on Two Problems in Connection with Graphs}},
    journal = "Numerische Mathematik",
    volume = "1",
    pages = "269-271",
    year = "1959",
}

@article{ccam97,
    author = "S. Shekhar and D. Liu",
    title = {{CCAM: A Connectivity-Clustered Access Method for Networks and Network Computations}},
    journal = "IEEE TKDE",
    volume = "19",
    number = "1",
    pages = "102-119",
    year = "1997",
}

@article{hepv,
author = "N. Jing and Y. W. Huang and E. A. Rundensteiner",
title = {{Hierarchical Encoded Path Views for Path Query Processing: An Optimal Model and Its Performance Evaluation}},
journal = "IEEE TKDE",
volume = "10",
number = "3",
pages = "409-432",
year = "1998",
}

@book{regression-book,
 author = {David Freedman},
 title = {{Statistical Models: Theory and Practice}},
 edition = {first},
 year = {2005},
 publisher = {Cambridge University Press},
}

@book{shashi,
 author = {Shashi Shekhar  and Sanjay Chawla},
 title = {{Spatial Databases: A Tour}},
 edition = {first},
 year = {2003},
 publisher = {Prentice Hall},
}


@book{voronoi-book,
 author = {A. Okabe and B. Boots and K. Sugihara and S. Chiu},
 title = {{Spatial Tessellations: Concepts and Applications of Voronoi Diagrams}},
 edition = {second},
 year = {2000},
 publisher = {Wiley},
}

@article{brinkhoff,
author = "T. Brinkhoff",
title = {{A Framework for Generating Network-based Moving Objects}},
journal = "GeoInformatica",
volume = "6",
number = "2",
pages = "153-180",
year = "2002",
}

@inproceedings{SJ-RTREE,
  author    = {T. Brinkhoff and H. Kriegel and B. Seeger},
  title     = {{Efficient processing of spatial joins using R-trees}},
  booktitle = sigmod,
  year      = {1993},
  pages={237--246}
  }

@article{multi-way,
 author = {N. Mamoulis and D. Papadias},
 title = {Multiway spatial joins},
 journal = tods,
 volume = {26},
 number = {4},
 year = {2001},
 pages = {424--475}
 }

@inproceedings{HashJoin,
  author    = {M.-L. Lo and C. V. Ravishankar},
  title     = {{Spatial hash-joins}},
  booktitle = sigmod,
  year      = {1996},
  pages={247--258}
  }


@inproceedings{Sweep,
  author    = {L. Arge and O. Procopiuc and S. Ramaswamy and T. Suel and J. Vitter},
  title     = {{Scalable sweeping-based spatial join}},
  booktitle = vldb,
  year      = {1998},
  pages={570--581}
  }

@inproceedings{mca06,
  author    = {Mohamed F. Mokbel and
               Chi-Yin Chow and
               Walid G. Aref},
  title     = {{The New Casper: Query Processing for Location Services without Compromising Privacy}},
  booktitle = {VLDB},
  year      = {2006},
  }

@inproceedings{ABGGKMMSTW04,
  author    = {Gagan Aggarwal and
               Mayank Bawa and
               Prasanna Ganesan and
               Hector Garcia-Molina and
               Krishnaram Kenthapadi and
               Nina Mishra and
               Rajeev Motwani and
               Utkarsh Srivastava and
               Dilys Thomas and
               Jennifer Widom and
               Ying Xu},
  title     = {{Vision Paper: Enabling Privacy for the Paranoids}},
  booktitle = {VLDB},
  year      = {2004},
  }

@inproceedings{aksx02,
  author    = {Rakesh Agrawal and
               Jerry Kiernan and
               Ramakrishnan Srikant and
               Yirong Xu},
  title     = {{Hippocratic Databases}},
  booktitle = {VLDB},
  year      = {2002},
  }


@inproceedings{ks04,
  author    = {Mohammad R. Kolahdouzan and Cyrus Shahabi},
  title     = {{Voronoi-Based K Nearest Neighbor Search for Spatial Network Databases}},
  booktitle = {VLDB},
  year      = {2004},
}

@inproceedings{jmw95,
  author    = {Nigel Jefferies and
               Chris J. Mitchell and
               Michael Walker},
  title     = {{A Proposed Architecture for Trusted Third Party Services}},
  booktitle = {Cryptography: Policy and Algorithms},
  year      = {1995},
  pages     = {98-104}
}

@inproceedings{pzmt03,
  author    = {Dimitris Papadias and
               Jun Zhang and
               Nikos Mamoulis and
               Yufei Tao},
  title     = {{Query Processing in Spatial Network Databases}},
  booktitle = {VLDB},
  year      = {2003},
}

@inproceedings{gks07,
  author    = {Gabriel Ghinita and
               Panos Kalnis and
               Spiros Skiadopoulos},
  title     = {{PRIVE: Anonymous Location-based Queries in Distributed Mobile Systems}},
  booktitle = {WWW},
  year      = {2007},
 }

@inproceedings{pkzt01,
  author    = {Dimitris Papadias and
               Panos Kalnis and
               Jun Zhang and
               Yufei Tao},
  title     = {{Efficient OLAP Operations in Spatial Data Warehouses}},
  booktitle = {SSTD},
  year      = {2001},
}

@article{tp03,
  author    = {Yufei Tao and
               Dimitris Papadias},
  title     = {{Spatial Queries in Dynamic Environments}},
  journal   = {ACM Trans. Database Syst.},
  volume    = {28},
  number    = {2},
  year      = {2003}
}

@article{sks03,
  author    = {Cyrus Shahabi and
               Mohammad R. Kolahdouzan and
               Mehdi Sharifzadeh},
  title     = {{A Road Network Embedding Technique for K-Nearest Neighbor
               Search in Moving Object Databases}},
  journal   = {GeoInformatica},
  volume    = {7},
  number    = {3},
  year      = {2003}
}

@article{kgmp07,
  author    = {Panos Kalnis and Gabriel Ghinita and Kyriakos Mouratidis and Dimitris Papadias},
  title     = {{Preserving Location-based Identity Inference in Anonymous Spatial Queries}},
  journal   = {IEEE TKDE},
  volume    = {19},
  number    = {12},
  year      = {2007}
}

@inproceedings{cml06,
  author    = {Chi-Yin Chow and
               Mohamed F. Mokbel and
               Xuan Liu},
  title     = {{A Peer-to-peer Spatial Cloaking Algorithm for Anonymous
               Location-based Service}},
  booktitle = {GIS},
  year      = {2006},
  pages     = {171-178}
}

@inproceedings{cm07,
  author    = {Chi-Yin Chow and
               Mohamed F. Mokbel},
  title     = {{Enabling Private Continuous Queries for Revealed User Locations}},
  booktitle = {SSTD},
  year      = {2007},
  pages     = {258-275}
}

@inproceedings{DVJPS03,
 author = {Ernesto Damiani and S. De Capitani Vimercati and Sushil Jajodia and Stefano Paraboschi and Pierangela Samarati},
 title = {{Balancing Confidentiality and Efficiency in Untrusted Relational DBMSs}},
 booktitle = {{Computer and Communications Security (CCS)}},
 year = {2003},
 pages = {93--102}
}

@inproceedings{YPPK08,
 author = {Yin Yang and Stavros Papadopoulos and Dimitris Papadias and George Kollios},
 title = {{Spatial Outsourcing for Location-based Services}},
 booktitle = {{ICDE}},
 year = {2008}
}

@inproceedings{GKKST08,
 author = {Gabriel Ghinita and Panos Kalnis and Ali Khoshgozaran and Cyrus Shahabi and Kian Lee Tan},
 title = {{Private Queries in Location Based Services: Anonymizers are not Necessary}},
 booktitle = sigmod,
 year = {2008}
}


@inproceedings{ko97,
  author    = {Eyal Kushilevitz and
               Rafail Ostrovsky},
  title     = {{Replication is NOT Needed: SINGLE Database, Computationally-Private
               Information Retrieval}},
  booktitle = {FOCS},
  year      = {1997},
}

@inproceedings{pir95,
  author    = {Benny Chor and
               Oded Goldreich and
               Eyal Kushilevitz and
               Madhu Sudan},
  title     = {{Private Information Retrieval}},
  booktitle = {FOCS},
  year      = {1995},
}



@inproceedings{BW07,
  author    = {Dan Boneh and Brent Waters},
  title     = {{Conjunctive, Subset, and Range Queries on Encrypted Data}},
  booktitle = {TCC},
  year      = {2007},
}

@inproceedings{GSW04,
  author    = {Philippe Golle and
               Jessica Staddon and
               Brent R. Waters},
  title     = {{Secure Conjunctive Keyword Search over Encrypted Data}},
  booktitle = {ACNS},
  year      = {2004},
}

@inproceedings{SBCSP07,
  author    = {Elaine Shi and
               John Bethencourt and
               Hubert T.-H. Chan and
               Dawn Xiaodong Song and
               Adrian Perrig},
  title     = {{Multi-Dimensional Range Query over Encrypted Data}},
  booktitle = {IEEE Symposium on Security and Privacy},
  year      = {2007},
}

@inproceedings{SWP00,
  author    = {Dawn Xiaodong Song and
               David Wagner and
               Adrian Perrig},
  title     = {Practical Techniques for Searches on Encrypted Data},
  booktitle = {IEEE Symposium on Security and Privacy},
  year      = {2000},
}

@article{bohm,
  title={{A Cost Model for Query Processing in High-Dimensional Data Spaces}},
  author={Christian B\"{o}hm},
  journal = {ACM TODS},
  volume={25},
  number={2},
  pages={129--178},
  year={2000}
}



@article{sam01,
  title={{Protecting Respondents' Identities in Microdata Release}},
  author={Samarati, P.},
  journal   = tkde,
  volume={13},
  number={6},
  pages={1010--1027},
  year={2001}
}

@inproceedings{gkkm07,
  author    = {Gabriel Ghinita and Panos Karras and
               Panos Kalnis and Nikos Mamoulis},
  title     = {{Fast Data Anonymization with Low Information Loss}},
  booktitle = {VLDB},
  year      = {2007}
 }

@inproceedings{xt07,
  author    = {Xiaokui Xiao and Yufei Tao},
  title     = {{m-invariance: towards privacy preserving re-publication of dynamic datasets}},
  booktitle = {SIGMOD},
  year      = {2007}
}


@inproceedings{ldr06,
  author    = {Kristen LeFevre and
               David J. DeWitt and
               Raghu Ramakrishnan},
  title     = {{Mondrian Multidimensional K-Anonymity}},
  booktitle = {ICDE},
  year      = {2006},
}

@inproceedings{ldr05,
  author    = {Kristen LeFevre and
               David J. DeWitt and
               Raghu Ramakrishnan},
  title     = {{Incognito: Efficient Full-Domain K-Anonymity}},
  booktitle = {SIGMOD},
  year      = {2005},
}

@MISC{AES,
  title =        {{Advanced Encryption Standard (AES)}},
  howpublished = {NIST - Federal Information Processing Standards Publication 197},
  year =         {2001},
  month =        {Nov},
}


@inproceedings{KYS05,
title={An anonymous communication technique using dummies for location-based services},
author={Kido, H. and Yanagisawa, Y. and Satoh, T.},
booktitle={International Conference on Pervasive Services (ICPS)},
year={2005},
pages={88-97}
}

@inproceedings{SpaceTwist,
title="{SpaceTwist: Managing the Trade-Offs Among Location Privacy, Query Performance, and Query Accuracy in Mobile Services}",
author={Man Lung Yiu and Jensen, C.S. and Xuegang Huang and Hua Lu},
booktitle={International Conference on Data Engineering (ICDE)},
year={2008},
pages={366-375}
}

@techreport{PROBE,
title="{PROBE: an Obfuscation System for the Protection of Sensitive Location Information in LBS}",
author={Maria Damiani and Elisa Bertino and Claudio Silvestri},
institution={CERIAS},
number={2001-145},
year={2008}
}

@inproceedings{CZBP06,
title="{Preserving User Location Privacy in Mobile Data Management Infrastructures}",
author={R. Cheng and Y. Zhang and E. Bertino and S. Prahbakar},
booktitle={Privacy Enhancing Technologies (PET)},
year={2006}
}



@inproceedings{Chor95,
    author = "Benny Chor and Oded Goldreich and Eyal Kushilevitz and Madhu Sudan",
    title = "Private Information Retrieval",
    booktitle = "{IEEE} Symposium on Foundations of Computer Science",
    pages = "41-50",
    year = "1995"
}

@inproceedings{Kushilevitz97,
    author = "Eyal Kushilevitz and Rafail Ostrovsky",
    title = "Replication is {NOT} Needed: Single Database, Computationally-Private Information Retrieval",
    booktitle = "{IEEE} Symposium on Foundations of Computer Science",
    pages = "364-373",
    year = "1997"
}

@article{Swe02,
    author = {Latanya Sweeney},
    title = "{k-Anonymity: A Model for Protecting Privacy}",
    journal = {Int. J. of Uncertainty, Fuzziness and Knowledge-Based Systems},
    year = {2002},
    volume = {10},
    number = {5},
    pages = {557-570}
}

@inproceedings{GG03,
  author    = {Marco Gruteser and
               Dirk Grunwald},
  title     = "{Anonymous Usage of Location-Based Services Through Spatial
               and Temporal Cloaking.}",
  booktitle = mobisys,
  year      = {2003}
}

@inproceedings{GL05,
  author    = {Bugra Gedik and
               Ling Liu},
  title     = "{Location Privacy in Mobile Systems: A Personalized Anonymization
               Model.}",
  booktitle = icdcs,
  year      = {2005},
  pages     = {620-629}
}


@inproceedings{Casper,
  author = {Mohamed F. Mokbel and Chi Yin Chow and Walid G. Aref},
  title = "{The New Casper: Query Processing for Location Services without Compromising Privacy}",
  booktitle = vldb,
  year = 2006,
}

@BOOK{ComGeometry,
  AUTHOR =       {Mark de Berg and Marc van Kreveld and Mark Overmars and Otfried Schwarzkopf},
  TITLE =        "{Computational Geometry: Algorithms and Applications}",
  PUBLISHER =    {Springer-Verlag},
  edition =      {2nd},
  YEAR =         {2000}
}

@INPROCEEDINGS{Cachin99,
    author = {Christian Cachin and Silvio Micali and Markus Stadler},
    title = {Computationally private information retrieval with polylogarithmic communication},
    booktitle = {EUROCRYPT},
    year = {1999},
    pages = {402--414},
    publisher = {Springer}
}

@inproceedings{SFBE07,
 author = {Monica Scannapieco and Ilya Figotin and Elisa Bertino and Ahmed K. Elmagarmid},
 title = {Privacy Preserving Schema and Data Matching},
 booktitle = sigmod,
 year = {2007},
 pages = {653--664}
}

@inproceedings{YAE09,
 author = {Mohamed Yakout and Mikhail Atallah and Ahmed Elmagarmid},
 title = {Efficient Private Record Linkage},
 booktitle = icde,
 year = {2009},
 pages = {1283--1286}
}

@inproceedings{AES03,
 author = {Rakesh Agrawal and Alexandre Evfimievski and Ramakrishnan Srikant},
 title = {Information Sharing Across Private Databases},
 booktitle = sigmod,
 year = {2003},
 pages = {86--97}
 }

@inproceedings{FNP04,
 author = {Michael J. Freedman and Kobbi Nissim and Benny Pinkas},
 title = {Efficient Private Matching and Set Intersection},
 booktitle = {Proc. of EUROCRYPT},
 year = {2004},
 pages = {1--19}
 }

@inproceedings{kissner,
    author = {Lea Kissner and Dawn Song},
    title = {Private and Threshold Set-Intersection},
    booktitle = {Proceedings of Annual International Cryptology Conference (CRYPTO)},
    year = {2005}
}


@inproceedings{Paillier,
    author = {Pascal Paillier},
    title = {Public-key cryptosystems based on composite degree residuosity classes},
    booktitle = {Proceedings of Annual Eurocrypt Conference (EUROCRYPT)},
    year = {1999},
    pages = {223--238}
}

@inproceedings{SSTD,
    author = {Gabriel Ghinita and Panos Kalnis and Murat Kantarcioglu and Eslisa Bertino},
    title = {A Hybrid Technique for Private Location-Based Queries with Database Protection},
    booktitle = sstd,
    year = {2009}
}

@inproceedings{inan:icde08,
  author    = {Ali Inan and
               Murat Kantarcioglu and
               Elisa Bertino and
               Monica Scannapieco},
  title     = {A Hybrid Approach to Private Record Linkage},
  booktitle = icde,
  year      = {2008},
  pages     = {496-505}
}


@article{SparseMap,
 author = {Hjaltason, G\'{\i}sli R. and Samet, Hanan},
 title = {Properties of Embedding Methods for Similarity Searching in Metric Spaces},
 journal = {IEEE Transactions on Pattern Analysys and Machine Intelligence},
 volume = {25},
 number = {5},
 year = {2003},
 pages = {530--549}
 }

 @inproceedings{gis10,
  author    = {Gabriel Ghinita and Carmen Ruiz Vicente and Ning Shang and Elisa Bertino},
  title     = {Privacy-preserving matching of spatial datasets with protection against background knowledge},
  booktitle = acmgis,
  year      = {2010},
  pages     = {3-12}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@INPROCEEDINGS{dmns06,
  AUTHOR =       {Cynthia Dwork and Frank McSherry and Kobbi Nissim and Adam Smith},
  TITLE =        {Calibrating Noise to Sensitivity in Private Data Analysis},
  BOOKTITLE =    {TCC},
  YEAR =         {2006},
  pages =        {265-284},
}


@INPROCEEDINGS{D10,
  AUTHOR =       {Cynthia Dwork},
  TITLE =        {Differential Privacy in New Settings},
  BOOKTITLE =    {SODA},
  YEAR =         {2010},
  pages =        {174-183},
}


@INPROCEEDINGS{ss98,
  AUTHOR =       {Pierangela Samarati and Latanya Sweeney},
  TITLE =        {Generalizing Data to Provide Anonymity when Disclosing Information (Abstract)},
  BOOKTITLE =    {PODS},
  YEAR =         {1998},
  pages =        {188},
}

@INPROCEEDINGS{mgkv06,
  AUTHOR =       {Ashwin Machanavajjhala and Johannes Gehrke and Daniel Kifer and Muthuramakrishnan Venkitasubramaniam},
  TITLE =        {$\ell$-Diversity: Privacy Beyond $k$-Anonymity},
  BOOKTITLE =    {ICDE},
  YEAR =         {2006},
  number =       {24},
}


%%%% NEW

@inproceedings{Boneh07,
 author = {Boneh, Dan and Waters, Brent},
 title = {Conjunctive, subset, and range queries on encrypted data},
 booktitle = {Proceedings of the 4th conference on Theory of cryptography},
 year = {2007},
 pages = {535--554}
} 

@article{Liu12,
 author = {Liu, Qin and Wang, Guojun and Wu, Jie},
 title = {Secure and privacy preserving keyword searching for cloud storage services},
 journal = {J. Network Computing Applications},
 volume = {35},
 number = {3},
 month = may,
 year = {2012},
 pages = {927--933}
} 

@inproceedings{Blundo09,
 author = {Blundo, Carlo and Iovino, Vincenzo and Persiano, Giuseppe},
 title = {Private-Key Hidden Vector Encryption with Key Confidentiality},
 booktitle = {Proceedings of the 8th International Conference on Cryptology and Network Security},
 year = {2009},
 pages = {259--277}
} 

@INPROCEEDINGS{Boneh06,
    author = {Dan Boneh and Amit Sahai and Brent Waters},
    title = {Fully Collusion Resistant Traitor Tracing with Short Ciphertexts and Private Keys},
    booktitle = {EUROCRYPT 2006, volume 4004 of LNCS},
    year = {2006},
    pages = {573--592}
}

@INPROCEEDINGS{Boneh03,
    author = {Dan Boneh and Giovanni Di Crescenzo and Rafail Ostrovsky and Giuseppe Persiano},
    title = {Public Key Encryption with Keyword Search},
    booktitle = {EUROCRYPT 2004, volume 3027 of LNCS},
    year = {2003}
}

@inproceedings{Boneh05,
 author = {Boneh, Dan and Goh, Eu-Jin and Nissim, Kobbi},
 title = {Evaluating 2-DNF formulas on ciphertexts},
 booktitle = {Proceedings of the Second international conference on Theory of Cryptography},
 year = {2005},
 pages = {325--341}
}

@inproceedings{espresso,
 author = {McGeer, Patrick and Sanghavi, Jagesh and Brayton, Robert and Vincentelli, Alberto Sangiovanni},
 title = {Espresso-signature: a new exact minimizer for logic functions},
 booktitle = {Proceedings of the 30th international Design Automation Conference},
 year = {1993},
 pages = {618--624}
}  

@article{quadtree,
 author = {Samet, Hanan},
 title = {The Quadtree and Related Hierarchical Data Structures},
 journal = {ACM Comput. Surv.},
 issue_date = {June 1984},
 volume = {16},
 number = {2},
 month = jun,
 year = {1984},
 pages = {187--260}
}

@article{Gray,
 author = {Bitner, James R. and Ehrlich, Gideon and Reingold, Edward M.},
 title = {Efficient generation of the binary reflected gray code and its applications},
 journal = {Commun. ACM},
 issue_date = {Sept. 1976},
 volume = {19},
 number = {9},
 month = sep,
 year = {1976},
 pages = {517--521}
} 

@article{Miller,
 author = {Miller, Victor S.},
 title = {The Weil Pairing, and Its Efficient Calculation},
 journal = {J. Cryptol.},
 issue_date = {September 2004},
 volume = {17},
 number = {4},
 month = sep,
 year = {2004},
 pages = {235--261}
}

@PHDTHESIS{pbc_thesis,
author = {Ben Lynn},
title = "{On the Implementation of Pairing-Based Cryptography}",
school = {Stanford University},
year=2007
}


@inproceedings{ks07,
  author    = {Ali Khoshgozaran and Cyrus Shahabi},
  title     = {{Blind Evaluation of Nearest Neighbor Queries Using Space Transformation to Preserve Location Privacy}},
  booktitle = {SSTD},
  year      = {2007},
}

@inproceedings{kido05,
 author = {H. Kido and Y. Yanagisawa and T. Satoh},
 title = {{An Anonymous Communication Technique using Dummies for Location-based Services}},
 booktitle = {IEEE International Conference on Pervasive Services (ICPS)},
 year = {2005},
}


@article{brinkhoff,
author = "T. Brinkhoff",
title = {{A Framework for Generating Network-based Moving Objects}},
journal = "GeoInformatica",
volume = "6",
number = "2",
pages = "153-180",
year = "2002",
}


@inproceedings{cml06,
  author    = {Chi-Yin Chow and
               Mohamed F. Mokbel and
               Xuan Liu},
  title     = {{A Peer-to-peer Spatial Cloaking Algorithm for Anonymous
               Location-based Service}},
  booktitle = {GIS},
  year      = {2006},
  pages     = {171-178}
}


@inproceedings{SpaceTwist,
title="{SpaceTwist: Managing the Trade-Offs Among Location Privacy, Query Performance, and Query Accuracy in Mobile Services}",
author={Man Lung Yiu and Jensen, C.S. and Xuegang Huang and Hua Lu},
booktitle={International Conference on Data Engineering (ICDE)},
year={2008},
pages={366-375}
}

@inproceedings{CZBP06,
title="{Preserving User Location Privacy in Mobile Data Management Infrastructures}",
author={R. Cheng and Y. Zhang and E. Bertino and S. Prahbakar},
booktitle={Privacy Enhancing Technologies (PET)},
year={2006}
}
@inproceedings{ks07,
  author    = {Ali Khoshgozaran and Cyrus Shahabi},
  title     = {{Blind Evaluation of Nearest Neighbor Queries Using Space Transformation to Preserve Location Privacy}},
  booktitle = {SSTD},
  year      = {2007},
}

@article{sec_priv,
 author = {M. Gruteser and X. Liu},
 title = {{Protecting Privacy in Continuous Location-Tracking Applications}},
 journal = {IEEE Security and Privacy},
 volume = {2},
 issue = {2},
 pages = {28-34},
 year = {2004}
}

@INPROCEEDINGS{expmech,
  AUTHOR =       {Frank McSherry and Kunal Talwar},
  TITLE =        {Mechanism Design via Differential Privacy},
  BOOKTITLE =    {Proc. of Annual IEEE Symposium on Foundations of Computer Science (FOCS)},
  YEAR =         {2007},
  pages =        {94-103}
}

@article{hcrmine,
  author = {M. Maruseac and G. Ghinita},
  title = {{Differentially-Private Mining of Moderately-Frequent
    High-Confidence Association Rules.}},
  journal = {{CODASPY Journal}},
  year = {2015}
}
@article{Kolonko,
	author = {Kolonko, M. and W\"{a}sch, D.},
	title = {Sequential Reservoir Sampling with a Nonuniform Distribution},
	journal = {ACM Trans. Math. Softw.},
	issue_date = {June 2006},
	volume = {32},
	number = {2},
	month = jun,
	year = {2006},
	issn = {0098-3500},
	pages = {257--273},
	numpages = {17},
	url = {http://doi.acm.org/10.1145/1141885.1141891},
	doi = {10.1145/1141885.1141891},
	acmid = {1141891},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Genetic algorithms, proportional selection, random sampling, reservoir sampling, roulette wheel simulation, sequential sampling},
}



@inproceedings{Katz:2008:PES,
	author = {Katz, Jonathan and Sahai, Amit and Waters, Brent},
	title = {Predicate Encryption Supporting Disjunctions, Polynomial Equations, and Inner Products},
	booktitle = {Proceedings of the Theory and Applications of Cryptographic Techniques 27th Annual International Conference on Advances in Cryptology},
	series = {EUROCRYPT'08},
	year = {2008},
	isbn = {3-540-78966-9, 978-3-540-78966-6},
	location = {Istanbul, Turkey},
	pages = {146--162},
	numpages = {17},
	url = {http://dl.acm.org/citation.cfm?id=1788414.1788423},
	acmid = {1788423},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
} 


@article{nakamoto2008bitcoin,
	title={Bitcoin: A peer-to-peer electronic cash system},
	author={Nakamoto, Satoshi},
	year = {2008}
}

@article{szabo1996smart,
	title={Smart contracts: building blocks for digital markets},
	author={Szabo, Nick},
	journal={EXTROPY: The Journal of Transhumanist Thought,(16)},
	year={1996}
}


